Adver-City: Open-Source Multi-Modal Dataset for Collaborative Perception Under Adverse Weather Conditions

Adverse weather conditions pose a significant challenge to the widespread adoption of Autonomous Vehicles (AVs) by impacting sensors like LiDARs and cameras. Even though Collaborative Perception (CP) improves AV perception in difficult conditions, existing CP datasets lack adverse weather conditions. To address this, we introduce Adver-City, the first open-source synthetic CP dataset focused on adverse weather conditions. Simulated in CARLA with OpenCDA, it contains over 24 thousand frames, over 890 thousand annotations, and 110 unique scenarios across six different weather conditions: clear weather, soft rain, heavy rain, fog, foggy heavy rain and, for the first time in a synthetic CP dataset, glare. It has six object categories including pedestrians and cyclists, and uses data from vehicles and roadside units featuring LiDARs, RGB and semantic segmentation cameras, GNSS, and IMUs. Its scenarios, based on real crash reports, depict the most relevant road configurations for adverse weather and poor visibility conditions, varying in object density, with both dense and sparse scenes, allowing for novel testing conditions of CP models. Benchmarks run on the dataset show that weather conditions created challenging conditions for perception models, with CoBEVT scoring 58.30/52.44/38.90 (AP@30/50/70). The dataset, code and documentation are available at https://labs.cs.queensu.ca/quarrg/datasets/adver-city/.

==> sec/4_benchmark_old.tex <==
\section{Benchmark}
\label{sec:benchmark}

How can a collaborative 3D object detection model trained without adverse weather generalize to adverse weather conditions? To answer that question, we used models trained on OPV2V \cite{xu_2021_opv2v} (which has no adverse weather) to perform inference on Adver-City, having as a baseline the Culver City testing scenario from OPV2V. 

We tested the trained baseline models provided by the authors of HEAL~\cite{lu_2024_heal} on Culver City, selecting the best-performing one for each sensor modality. Since the models for camera-based detection were trained with depth data, they were disregarded from our analysis as the removal of depth made the models unsuitable for detection (the top camera-based model achieved an AP@$50$ of $19.02$). Both for LiDAR and LiDAR + Camera detection, CoBEVT~\cite{xu_2022_cobevt} was the best model for Culver City and was then used for inference in the Adver-City scenarios presented in Table~\ref{tab:benchmark}. PointPillars~\cite{lang_2019_pointpillars} was used as the backbone for LiDAR models, and Lift-Splat-Shoot~\cite{phillion_2020_lift}, with EfficientNet~\cite{tan_2019_efficientnet} as the image encoder, was used for camera experiments. All Adver-City experiments were conducted across the five road configurations described in Section~\ref{subsec:scenarios}.

Even though our dataset follows the OPV2V annotation schema, minor adjustments were required to ensure the OPV2V-trained model performed adequately on Adver-City. Since OPV2V includes only the `car' category, the model was limited to detecting cars. Bounding boxes for dissimilar categories such as `pedestrian', `bicycle', and `motorcycle', were removed for the benchmark. Also, data from RSUs was excluded since OPV2V does not support V2X collaboration.

\begin{table*}%[!thb]
\centering
\begin{tabular}{cc|clcl|clcl}
\toprule
\multirow{3}{*}{\textbf{Dataset}} & \multirow{3}{*}{\parbox[c]{.1\linewidth}{\centering \textbf{Scenario}}} & \multicolumn{4}{c|}{\textbf{Lidar (AP@50)}} & \multicolumn{4}{c}{\textbf{Lidar + Camera (AP@50)}} \\ \cmidrule{3-10} 
    & & \multicolumn{2}{c}{Day}   & \multicolumn{2}{c|}{Night}& \multicolumn{2}{c}{Day}   & \multicolumn{2}{c}{Night}    \\ \cmidrule{3-10} 
    & & Sparse & \multicolumn{1}{c}{Dense} & Sparse& \multicolumn{1}{c|}{Dense} & Sparse   & \multicolumn{1}{c}{Dense}    & Sparse  & \multicolumn{1}{c}{Dense}   \\ \midrule
\multirow{6}{*}{Adver-City}   & Clear Weather  & $53.22$  & $44.49$  & $54.19$ & $44.95$   & $46.70$    & $41.53$ & $42.76$ & $39.50$    \\
    & Soft Rain         & $52.50$ & $43.73$  & $53.80$ & $42.32$ & $42.30$ & $40.45$ & $39.42$ & $34.78$    \\
    & Heavy Rain        & $54.38$ & $42.05$  & $49.42$ & $44.71$ & $43.06$ & $38.72$ & $34.11$ & $38.03$    \\
    & Fog& $52.98$ & $43.24$  & $52.81$ & $40.04$ & $38.68$ & $36.68$ & $37.55$ & $34.11$    \\
    & Foggy Heavy Rain  & $54.31$ & $42.97$  & $54.42$ & $38.76$ & $37.83$ & $35.77$ & $40.40$ & $34.18$    \\
    & Glare             & $53.71$ & $42.29$  & \multicolumn{2}{c|}{-} & $42.43$  & $38.55$ & \multicolumn{2}{c}{-}   \\ \midrule
OPV2V \cite{xu_2021_opv2v} & Culver City & \multicolumn{2}{c}{$79.52$} & \multicolumn{2}{c|}{-} & \multicolumn{2}{c}{$70.27$} & \multicolumn{2}{c}{-}   \\ \bottomrule
\end{tabular}
\caption{Benchmark results from collaborative 3D object detection models trained on OPV2V and tested with unseen data. All experiments used CoBEVT \cite{xu_2022_cobevt} models provided by the authors of HEAL \cite{lu_2024_heal}. PointPillars \cite{lang_2019_pointpillars} was used as the backbone for Lidar, while Lift-Splat-Shoot \cite{phillion_2020_lift} was used for camera with EfficientNet \cite{tan_2019_efficientnet} as the image encoder. While Lidar experiments were more influenced by object density, Lidar + Camera experiments were more influenced by adverse weather conditions.}
\label{tab:benchmark}
\end{table*}

The average performance drop between Adver-City and Culver City ($31\%$ for both modalities) was due to differences in sensor configurations, positioning, and scenario locations. Despite this, clear patterns emerged: LiDAR-based detection was less impacted by adverse weather ($3.9\%$ variation between weather conditions, on average) than LiDAR + Camera ($7.2\%$ variation). On the other hand, LiDAR-based detection was more affected by higher object density ($10.6\%$ variation) than LiDAR + Camera ($3.0\%$ variation). 

Despite CARLA's limitations, performance noticeably dropped as weather conditions became more challenging, with a $19\%$ decline for the LiDAR + Camera model on sparse day scenarios. Moreover, the results highlight the diversity of Adver-City's scenarios, with a performance gap of nearly $29\%$ for LiDAR-based detection and $27\%$ for LiDAR + Camera between the highest- and lowest-scoring scenarios.

Since camera-based 3D object detection was not viable with HEAL's models, we performed 2D object detection with YOLOv8~\cite{qiu_2023_yolov8} trained on the COCO dataset~\cite{lin_2015_coco} to assess the impact of adverse weather on camera-based detection. The detection was done using only the front-facing camera of the ego vehicle. As shown in Table~\ref{tab:yolo}, the model performed slightly below the baseline YOLO models on similar weather conditions, with results being impacted by nighttime by almost $26\%$.

\begin{table}
\centering
\resizebox{0.49\textwidth}{!}{\begin{tabular}{c|cccc|c}
\toprule
\multirow{3}{*}{\textbf{Scenario}} & \multicolumn{4}{c|}{\textbf{Camera (mAP50)}}         & \multirow{2}{*}{\textbf{Baseline}} \\ \cmidrule{2-5}
& \multicolumn{2}{c}{Day} & \multicolumn{2}{c|}{Night} & \textbf{(Day)} \\ \cmidrule{2-5}
& S          & D          & S            & D           & \\ \midrule
Soft Rain           & $46.7$       & $44.4$       & $33.9$         & $35.1$        & $57.1$~\cite{kim_2023_challenges} \\
Heavy Rain          & $42.1$       & $41.8$       & $21.5$         & $27.7$        & $46.0$~\cite{kim_2023_challenges} \\
Fog  & $48.6$       & $41.4$       & $42.1$         & $34.2$        & $53.6$~\cite{chu_2024_dyolo} \\
Foggy Heavy Rain    & $38.7$       & $40.9$       & $34.4$         & $26.7$        & -          \\
Glare& $38.7$       & $38.9$       & \multicolumn{2}{c|}{-}     & -          \\ \bottomrule
\end{tabular}}
\caption{Benchmark results from 2D object detection performed with YOLOv8~\cite{qiu_2023_yolov8} on Adver-City's adverse weather scenarios. S: sparse, D: dense. While glare was the most challenging condition for daytime scenarios, heavy rain was the toughest for nighttime.}
\label{tab:yolo}
\end{table}

Standing out from the 3D object detection benchmarks, object density played a lesser role in 2D object detection, with the median result being very similar both for sparse ($38.7$) and dense ($38.9$) scenarios, which is caused by different annotation strategies between the two tasks. While occlusion may heavily impact 3D detection, it is less prevalent in 2D detection because a completely occluded object will not have a corresponding 2D bounding box. Therefore, even when using 2D object detection techniques, it might be important to correlate different cameras -- from the ego vehicle, the connected vehicles, and the RSUs -- for improved detection. This is a new avenue of research that can be explored with Adver-City.
